Ergonomic-driven Geometric Exploration and Reshaping

The paper addresses the following problem: given a set of man-made shapes, e.g., chairs, can we quickly rank and explore the set of shapes with respect to a given avatar pose? Answering this question requires identifying which shapes are more suitable for the defined avatar and pose; and moreover, to provide fast preview of how to alter the input geometry to better fit the deformed shapes to the given avatar pose? The problem naturally links physical proportions of human body and its interaction with object shapes in an attempt to connect ergonomics with shape geometry. We designed an interaction system that allows users to explore shape collections using the deformation of human characters while at the same time providing interactive previews of how to alter the shapes to better fit the user-specified character. We achieve this by first mapping ergonomics guidelines into a set of simultaneous multi-part constraints based on target contacts; and then, proposing a novel contact-based deformation model to realize multi-contact constraints. We evaluate our framework on various chair models and validate the results via a small user study.

==> related_work.tex <==
\section{Related Work}
Our work is closely related to existing works on shape exploration, geometric classification, and ergonomics study. While previous approaches exploit purely geometric or learning-based methods to achieve shape understanding, we focus on ergonomics both for classification and geometric deformation. %Here we briefly review the relevant literature.

\mypara{Shape exploration}
%As the online repositories of 3{D} models continue to expand, effective browsing the large collections of shape data is demanding.
Recent research has proposed shape exploration tools to allow users to quickly browse large data collections. These methods either provide fast previews of shape variations \cite{Ovsjanikov11}, find partial correspondence \cite{Kim13}, or organize shapes into collective structures \cite{huang2013quartet}. The methods start from a pure geometric point of view to extract commonalities among a family of shapes using geometric descriptors or functional maps to find shape similarity. In contrast, we relate ergonomics with geometry to measure inter- and intra-class similarity for a given shape collection.


\mypara{Shape functional analysis}
Functionality of objects is closely related to their semantics. Understanding the shape functional properties remains the central challenge of existing shape analysis techniques. In recent years, a few methods have been proposed to reveal such connections based on purely geometry-based attempts \cite{laga_acmtog2013,Zheng:2014}. These approaches start from component-level models and build part-level contact graphs to facilitate subsequent analysis. In comparison, we exploit ergonomics guidelines to leverage a graph representation for the part-level deformation.


\mypara{Geometry and human factor}
Geometry reasoning has also been studied in computer vision and used for human workspace reasoning \cite{Fouhey12} or indoor scene understanding \cite{Gupta_CVPR11}. While these methods uses extensive training from existing semantic measures of image data to reason about a given particular image, the process of human measurement is typically performed offline. Coupling geometry modeling with physical simulation has been studied in recent research work of interactive chair modeling \cite{Saul:2010:SAC}. For an extensive discussion of history and development of
 ergonomics in the context of chairs we recommend Cranz's book~\cite{book88}, especially Chapters 3 and 5.


\mypara{Shape deformation}
Shape deformation has been a long-standing research topic in geometry processing \cite{DeformationSurvey:2008}. Existing shape deformation methods mainly fall into two classes: one class of methods aim to preserve the shape local properties such as curvatures, local coordinates, etc., \cite{Sorkine:2004,Lipman:2005:LRC,Lipman:2008:GC}, while the other class of methods aim to preserve global structures such as symmetry, inter-part relations \cite{Kraevoy:2008,Gal2009,ZFDOT10}.
%
Li et al.~\shortcite{Li_siga12}, in an interesting work, deforms input man-made objects to make them amendable to stacking.
%
In contrast, we focus on ergonomics guidelines for customizing chairs and sofas for specific target avatar sizes and poses. %The key enabler to our deformation framework is a set of contacts that connect the shape components and link the structural relations of the shape.



